MMCBE: Multi-modality Dataset for Crop Biomass Prediction and Beyond

Crop biomass, a critical indicator of plant growth, health, and productivity, is invaluable for crop breeding programs and agronomic research. However, the accurate and scalable quantification of crop biomass remains inaccessible due to limitations in existing measurement methods. One of the obstacles impeding the advancement of current crop biomass prediction methodologies is the scarcity of publicly available datasets. Addressing this gap, we introduce a new dataset in this domain, i.e. Multi-modality dataset for crop biomass estimation (MMCBE). Comprising 216 sets of multi-view drone images, coupled with LiDAR point clouds, and hand-labelled ground truth, MMCBE represents the first multi-modality one in the field. This dataset aims to establish benchmark methods for crop biomass quantification and foster the development of vision-based approaches. We have rigorously evaluated state-of-the-art crop biomass estimation methods using MMCBE and ventured into additional potential applications, such as 3D crop reconstruction from drone imagery and novel-view rendering. With this publication, we are making our comprehensive dataset available to the broader community.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/1_intro_05_11.tex <==
\section{Introduction}
\label{sec:intro}

Story-line: biomass prediction is an important task, but there is a lack of a unified benchmark with a public-available dataset for algorithm comparison, also all approaches focus on utilizing LiDAR point cloud rather than computer vision which has the potential to be applied in a larger scale and has a more widespread impact in agriculture. Therefore, we are going to present a benchmark and public-available dataset for biomass prediction tasks and this dataset includes both point cloud and image sets, which can provide an evaluation for various biomass-prediction approaches. Besides, we propose two different methods for point-cloud-based and vision-based methods respectively, which provide a strong baseline for the other methods.
\begin{itemize}
  \item Proposing a sparse 3D CNN + transformation feature, which is demonstrated on biomass prediction method task;
  \item Proposing a vision-based biomass prediction method (the same as above); 
  \item Training on pseudo point cloud, generated from point cloud, evaluated on real LiDAR point cloud.
  \item To validate our proposed methods, publishing benchmark with a public-available dataset for biomass prediction task, and the dataset includes both point cloud and images.
  \item A new data augmentation to enlarge the data sample; (Random sample splitting and combination)
\end{itemize}


\textcolor{red}{TODO: is there a way to regularize a single-value prediction? is there a way to improve the Sparse+Vit framework?}
\begin{itemize}
  \item Adding auxiliary task, like semantic segmentation loss
  \item Adding biomass prediction with uniform distribution
\end{itemize}


==> sec/1_intro_17_11.tex <==
\vspace*{-\baselineskip}

\section{Introduction}
\label{sec:intro}

The amount of organic matter a plant produces is called biomass. In this paper, the term 'biomass' specifically refers to above-ground biomass (ie. excluding roots). Biomass is a key trait to monitor agricultural systems, being used to determine the success of plant establishment and inform decisions around replanting, or to apply a range of treatments such as chemical sprays. It is also a key parameter to determine which plants to select in crop breeding programs. Having access to this valuable trait helps to increase agricultural production and confront global agricultural challenges such as feeding the ever-increasing world population~\cite{united2019certain}. Unfortunately, measuring this trait accurately and at scale is currently impractical due to the limitations of existing methods \cite{pan2022biomass, loudermilk2009ground}. 

Conventional biomass quantification relies on harvesting and measuring the biomass of a small plot area (eg. a square meter or a linear meter) and relating this value to a whole plot or field. This approach is a destructive and laborious approximation, which means it does not scale and cannot be used to generate temporal data. On the contrary, computer vision offers the opportunity to non-destructively measure biomass through time \cite{walter2019estimating, jimenez2018high, caballer2021prediction, sun2018field, polo2009tractor, ten2019biomass, pan2022biomass}.  LiDAR in particular has been used to capture plant height and point density, serving as a proxy to estimate biomass.  Proxy-based methods tend to be generalizable, but their simple 3D feature representation and canopy self-occlusion limit their accuracy. To further improve estimation accuracy, deep learning mechanisms have been introduced to address the issue of self-occlusion and learn strong 3D features from point clouds~\cite{pan2022biomass}. However, the current deep learning-based method still suffers the low accuracy due to ineffective 3D feature extraction and limited dataset. To address this, we propose to build a generalized biomass backbone network (Generalized BioNet) to improve the prediction accuracy. The generalized BioNet mainly consists of sparse 3D CNN operations in the point cloud and it can inherently gain the benefits of translation invariance, exploitation of spatial structure, and parameter sharing and reduction CNN~\cite{NIPS2012_c399862d, lecun1998gradient} 
 which can improve the generalization capability beyond a small dataset.

CNN~\cite{NIPS2012_c399862d, lecun1998gradient} over MLP parameter sharing and reduction (increasing generalization capability of the model over small dataset), exploitation of spatial structure. translation invariance, and hierarchical feature learning. When collecting and processing the crop dataset for the biomass prediction task, the sensor looks downward and scans the crops with more translation and less rotation. This pattern makes the CNN a more suitable choice for the backbone network, due to its feature of rotation invariant. 





However, the requirement for high-resolution LiDAR point cloud data constrains the scalability of these approaches to large fields. Vision-based biomass measurement methods (ie. those relying on RGB imaging) are particularly appealing due to the widespread availability and affordability of RGB cameras. These methods typically reconstruct 3D pseudo point clouds using multi-view images through structure-from-motion (SfM)~\cite{schonberger2016structure, ye2023uav, Alonzo_2020, schoenberger2016mvs}, and then apply aforementioned proxy-based methods to predict biomass. However, their prediction accuracy is limited by the 3D reconstruction performance and simple 3D features. To push vision-based methods further, in this study we introduce 'NeFF-BioNet', a novel multi-view image-based biomass estimation neural network consisting of two modules: NeFF and BioNet. The NeFF module is designed to extract 3D features from multi-view images, using neural implicit fields to learn the geometry, radiance, and semantic features of a plant plot. Specifically, NeFF reconstructs 3D plants from the neural geometry field and scatters semantic features from the learned feature field to the reconstructed 3D plant surface. Subsequently, the BioNet module takes the extracted 3D features as input for a sparse 3D CNN backbone to further refine 3D features and compress them into 2D feature maps. To predict biomass from these feature maps, we employed current state-of-the-art (SOTA) Transformer encoders\cite{vaswani2017attention}. Experimental results demonstrate that our NeFF-BioNet achieves about 18\% accuracy gains over the SOTA methods. To the best of our knowledge, this represents the first vision and learning-based biomass estimation method with the potential for large-scale application. Our key contributions are summarized as follows:
\begin{itemize}
  \item We have introduced a point-supervised neural feature field that effectively completes three tasks: 3D reconstruction, semantic feature distillation, and novel-view image synthesis.
  \item We have developed a novel vision-based neural network architecture named 'NeFF-BioNet', which not only achieves higher prediction accuracy compared to current biomass measurement methods but also has the potential to scale to large fields.
  \item We are publishing the dataset we collected to create NeFF-BioNet, namely a set of 216 multi-view drone image sets with their hand-labeled ground truth. This dataset will help the community to establish benchmark methods to quantify plant biomass.
\end{itemize}


==> sec/3_method_17_11.tex <==
\begin{figure*}[htb]
    \centering
    \includegraphics[width=1.8\columnwidth]{figs/NeFF.pdf}
    \caption{The framework of our NeFF module. The neural geometry field ${F}_{g}$ takes as input the sampled points $\mathbf{x}$ along camera ray $\mathbf{r}(t)$ (red arrow) and sparse points $\textbf{P}^{S}$ from SfM. The red cuboid represents SDF output for points belonging to $\textbf{P}^{S}$. The white cuboid denotes geometry features, based on which the implicit neural feature field ${F}_{f}$ predicts the 3D semantic features for points $\mathbf{x}$. The neural radiance field ${F}_{c}$ will predict the colors of sampled 3D points $\mathbf{x}$ with viewing direction $\mathbf{v}$. The novel-view image and its feature maps are rendered through the volumetric rendering with NeuS volumetric density function \cite{NeuS_3D_reconstru}. Our NeFF is optimized with three loss functions.}
    \label{fig:NeFF}
\end{figure*}


%%%%%%%%% BODY TEXT
\section{Neural feature field}
\label{sec:NeFF}

Given multi-view images of a static scene $(I_{1}, I_{2}, \ldots, I_{n})$, $I_i \in \mathbb{R}^{3 \times H \times W}$, neural feature field is to distill 2D features extracted by foundation models from them into a 3D representation for the biomass prediction module. These 3D features should not only encode generalized semantic content, which aid in distinguishing different plant parts and in isolating them from the ground, but also capture the 3D spatial plant structure. 

\subsection{Neural implicit scene representation}
The scene of the object can be separated into two fundamental aspects: geometry and appearance. Similar to NeuS \cite{NeuS_3D_reconstru}, we represent the geometry of the scene using a neural implicit surface with SDF, due to its enhanced 3D reconstruction with a better decoupling between the geometry and appearance information \cite{yariv2020multiview, NeuS_3D_reconstru, yariv2021volume}. Given a 3D location $\textit{\textbf{x}} = (x,y,z) \in \mathbb{R}^{3}$ in the specified 3D volume, the geometry mapping function, i.e. SDF, is defined as ${F}_{g}: \textit{\textbf{x}} \longrightarrow \textit{s} $, and $s \in \mathbb{R}$ is the signed distance of \textbf{x} to the object's surface, approximated by a multi-layer perception (MLP). The surface $\textit{S}$ of the object is depicted by the zero-level set of its SDF as follows:
\begin{equation}
\begin{aligned}
 \textit{S} = \{ \textbf{\textit{x}} \in \mathbb{R}^{3} | {F}_{g}(\textbf{\textit{x}}) = 0 \}
\label{equ:sdf}
\end{aligned}
\end{equation}

The appearance, i.e. radiance field, is represented by another independent MLP, and the color mapping function is $F_{c}: (\mathbf{x}, \mathbf{v}) \longrightarrow \mathbf{c}$. Since the appearance is view-dependent, the viewing direction $\mathbf{v} \in \mathbb{R}^{2}$ is included in the input. The output $\mathbf{c} \in \mathbb{R}^{3}$ (RGB) represents the color emitted from point $\mathbf{x}$ along the viewing direction $\mathbf{v}$. After getting both the geometry and appearance, volume rendering is applied to generate image colors. Given a camera ray $\mathbf{r}(t) = \mathbf{o} + t\mathbf{v}$, where $\mathbf{o}$ is the camera origin, the expected color of this ray is the integrated color along the ray with near ($t_{\text{n}}$) and far ($t_{\text{f}}$) bounds. This integration can be expressed as follows:
\begin{equation}
\begin{aligned}
\mathbf{\hat{c}(r)} =  \int_{t_{\text{n}}}^{t_{\text{f}}} w(t)\mathbf{c}(\mathbf{x}(t), \mathbf{v})dt  =   \int_{t_{\text{n}}}^{t_{\text{f}}} w(t){F}_{c}(\mathbf{x}(t), \mathbf{v})dt
\label{equ:volume}
\end{aligned}
\end{equation}
\noindent where $\mathbf{x}(t)$ is sampled 3D point along ray $\mathbf{r}$ at $t$ positon and $w(t)$ is its integration weight. The $w(t)$ is calculated by multiplying volume density $\sigma(t)$ and accumulated transmittance \textit{T(t)}, as following equation:
\begin{equation}
\begin{aligned}
% & w(t) = \textit{T(t)}\sigma(t) \\
% & T(t) = exp(-\int_{t_{\text{n}}}^{t} \sigma(s) ds)
w(t) = \textit{T(t)}\sigma(t), T(t) = exp(-\int_{t_{\text{n}}}^{t} \sigma(s) ds)
\label{equ:weight}
\end{aligned}
\end{equation}
\noindent To establish the connection between  SDF ${F}_{g}(t)$ and volume density $\sigma(t)$, the following volumetric density function~\cite{NeuS_3D_reconstru} is used to map them:
\begin{equation}
\begin{aligned}
\sigma(t) = max \left( \frac{-\frac{\Phi}{\text{d}t}({F}_{g}(\mathbf{x}(t)))}{\Phi({F}_{g}(\mathbf{x}(t)))},0  \right)
\label{equ:density}
\end{aligned}
\end{equation}
\noindent where $\Phi(x)$ is the sigmoid function. This approximated function $\sigma(t)$ has unbiased and occlusion-aware properties, the detailed proof can refer to the papers \cite{NeuS_3D_reconstru, mildenhall2021nerf}. After combining equation \ref{equ:weight} and \ref{equ:density}, we can derive the weight $w(t)$ from SDF ${F}_{g}(t)$. With the geometry and appearance information, we are able to synthesize an image of the scene from any novel view via volume rendering. %The integration is practically approximated with a numerical quadrature on a set of sampled points along the camera ray.

\label{sec:BPN}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=1.8\columnwidth]{figs/bionet.pdf}
    \caption{The framework of the biomass prediction module, BioNet. A sparse 3D CNN backbone further refines and extracts 3D features generated by the NeFF module. The final 2D feature map is flattened into a feature embedding, to which a learnable biomass embedding token (yellow cuboid) is appended. The biomass token serves as an overall 3D feature representation and is connected with a two-layer MLP to predict the final biomass. The feature embedding is added to the learnable position embedding before the transformer encoder. The rightmost panel shows the structure of the Transformer encoder as inspired by \cite{vaswani2017attention}}
    \label{fig:bpn}
\end{figure*}

\subsection{Semantic feature representation}
\label{sec:feature_field_rep}
To generate a continuous 3D semantic feature volume, we use a neural feature field to distill the knowledge from the 2D foundation model, DINO \cite{caron2021emerging}, via neural rendering. The 2D foundation model, trained on the large image dataset, generally has a strong generalization capability \cite{oquab2023dinov2}, and the distilled knowledge can help to overcome the shortage of labeled data in the domain dataset. The extracted features from the foundation model for each image are $(F_{1}, F_{2}, \ldots, F_{n}), F_i \in \mathbb{R}^{c \times h \times w}$, where $c$ is the feature dimension. The semantic feature field is view-independent, and its mapping function can be defined as $F_{f}: \mathbf{x} \longrightarrow \mathbf{f}$, where $\mathbf{f} \in \mathbb{R}^{c}$. Similar to learning the radiance field via rendering color, We learn the feature field $F_{f}$ by the volumetric rendering of the 2D feature map $F_i$. Therefore, the expected 2D feature for a camera ray, $\mathbf{r}(t) = \mathbf{o} + t\mathbf{v}$, can be represented as equation \ref{equ:feature}, in which the scene geometry $w(t)$ is the same to equation \ref{equ:volume}.
\begin{equation}
\begin{aligned}
\mathbf{\hat{f}(r)}  = \int_{t_{\text{n}}}^{t_{\text{f}}} w(t)\mathbf{f}(\mathbf{x}(t))dt =   \int_{t_{\text{n}}}^{t_{\text{f}}} w(t){F}_{f}(\mathbf{x}(t))dt
\label{equ:feature}
\end{aligned}
\end{equation}
\subsection{Loss function}
If three neural representation functions (i.e. $F_{g}$, $F_{c}$, and $F_{f}$) are well learnt, we should be able to render both image and feature map with high-fidelity. Therefore, given a camera ray $\mathbf{r}$, we can construct the color loss function to minimize the difference between the rendered image $\hat{\mathbf{c}}(\mathbf{r})$ and ground truth one $\mathbf{c}(\mathbf{r})$, as following equation.
\begin{equation}
\begin{aligned}
 \mathcal{L}_{c} =  \sum_{\mathbf{r} \in \mathbf{R}} || \hat{\mathbf{c}}(\mathbf{r}) - \mathbf{c}(\mathbf{r}) ||
\label{equ:loss_color}
\end{aligned}
\end{equation}
\noindent where $\mathbf{R}$ is the sampled rays for training. Similarly, the feature loss function can be built to optimize function $F_{f}$. 
\begin{equation}
\begin{aligned}
 \mathcal{L}_{f} =  \sum_{\mathbf{r} \in \mathbf{R}} || \hat{\mathbf{f}}(\mathbf{r}) - \mathbf{f}(\mathbf{r}) ||
\label{equ:loss_feature}
\end{aligned}
\end{equation}
In practice, we find that these two losses are not strong enough to recover the geometry information, seeing Fig. \ref{fig:depth}. This can be caused by two reasons, one is that plants are quite small and most area in the scene is quite boring and flat, other is that the $F_{g}$ is implicitly learned with color and features with direct supervision. Given multi-view images, we run the SfM \cite{schonberger2016structure} to obtain the camera parameters, and a sparse point cloud is generated as a side-product. To better optimize the $F_{g}$, we use this sparse point cloud to directly optimize $F_{g}$. The constructed loss is as follows:
\begin{equation}
\begin{aligned}
 \mathcal{L}_{g} =  \sum_{\mathbf{x} \in \mathbf{P}^{S}} || {F}_{g}(\mathbf{x}) - 0 ||
\label{equ:loss_geometrical}
\end{aligned}
\end{equation}
\noindent where $\mathbf{P}^{S} \in \mathbb{R}^{k \times 3}$ is denoted as the sparse point cloud from SfM and $k$ is the number of points. The final loss function for optimizing the NeFF is as follows:
\begin{equation}
\begin{aligned}
 \mathcal{L}_{NeFF} =  \mathcal{L}_{f} + \alpha \mathcal{L}_{c} + \beta \mathcal{L}_{g}
\label{equ:loss_totall}
\end{aligned}
\end{equation}

\section{Biomass prediction network}
We exploited the power of Transformers~\cite{vaswani2017attention, dosovitskiy2020image} for biomass prediction and introduced a hybrid architecture, as shown in Fig. \ref{fig:bpn}, in which a 3D sparse CNN was employed to reduce the 3D semantic features generated by the NeFF module into lower dimensions. Their spatial dimensions were then flattened to form a feature sequence used as the Transformer input. 

\subsection{3D feature extraction}
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.76\columnwidth]{figs/3DBN.pdf}
    \caption{Architecture of the sparse 3D CNN backbone. The input is the voxelized 3D features generated from NeFF. SSCNN stands for submanifold sparse 3D CNN\cite{graham2017submanifold}, while SCNN stands for sparse 3D CNN. Each pyramidal level consists of two ResNet blocks \cite{he2016identity}.}
    \label{fig:3dbn}
\end{figure}
The distilled feature field from the vision model generally contains more semantic features than spatial structures and it is necessary to use a 3D backbone, mainly consisting of sparse 3D CNN layers, to extract 3D geometric features. Sparse 3D CNN takes advantage of spatial sparsity in point cloud data \cite{s18103337, li2019three}, which can significantly reduce memory and processing costs when extracting 3D features. The feature field takes as input a 3D grid position and outputs its semantic features, so the 3D semantic features can have any high resolution, and we initially sampled high-resolution 3D grids with Equ.\ref{equ:sdf} to generate the surface points and their semantic features. The input points were assumed to be $\mathbf{P}^{f} \in \mathbb{R}^{n \times (3+c)}$, where $n$ denotes the number of sampled surface points (usually millions), $c$ is the feature channel number, and 3 represents its location dimension. The sparse 3D CNN expects its input to be organized within a regular grid, but the point cloud data is usually in an irregular format. We therfore first voxelized the $\mathbf{P}^{f}$ to obtain its voxel representation. Each resulting voxel may contain several points, so we averaged all points inside a given voxel to obtain its final feature. Our resulting voxelized feature map with high resolution equates to $l^v \times w^v \times h^v \times (3+c)$. In our application, $h$ is usually the lowest number. Each feature map was then processed by separate sparse 3D CNN blocks to generate the 3D features. We used a regular $3 \times 3\times 3$ convolutional kernel and submanifold CNN \cite{graham2017submanifold} without max pooling until the 3D feature map became 2D, i.e. $h$ dimension becomes 1. The network architecture is shown in Fig. \ref{fig:3dbn}.

\subsection{Transformer for biomass prediction}
Transformer architecture has become very successful in various computer vision tasks \cite{carion2020end, dosovitskiy2020image, vaswani2017attention} due to its strong capability in feature extraction, and were therefore explored for our application. After getting the final feature from 3D sparse CNN, we flattened the feature map $\mathbf{V}^{t} \in \mathbb{R}^{h^t \times w^t \times c^t}$ into a 1-dimensional token sequence $\mathbf{V}^{t}_1 \in \mathbb{R}^{(h^t\times w^t) \times c^t}$ as the input for the Transformer. Similar to \texttt{Class} token in ViT \cite{dosovitskiy2020image}, we prepended a learnable embedding, called \texttt{Biomass} token, to the feature embedding $\mathbf{V}^{t}_1$. The \texttt{Biomass} token serves as the 3D feature representation for the entire scene and interacts with overall spatial features. It can be treated as an agent extracting or summarizing all feature embeddings. Position embeddings are added to each feature embedding to retain positional information. We used standard learnable 1D position embedding \cite{vaswani2017attention}. The resulting sequence of embedding vectors was used as input for Transformer encoders. A biomass prediction head with two-layers MLP was connected with the \texttt{Biomass} token for the final prediction. The prediction biomass value is $\hat{m}$, and the final biomass prediction loss was calculated as follows:
\begin{equation}
\begin{aligned}
\mathcal{L}_{b} =  \sum_{i=1}^{N} \mathrm{f} \left( \frac{\hat{m}_i - m_i}{\log(m_i)} \right)
\label{equ:bio_pred}
\end{aligned}
\end{equation}
\noindent where $m_i$ is the corresponding ground truth, and smooth $\boldsymbol\ell$1 loss function, $\mathrm{f}$ \cite{smoothl1}, was used to calculate the final prediction loss. To address the issue of the large varying ranges of biomass ground truth throughout the season, we regularized the residue between prediction and ground truth using $\log(m_i)$, resulting in a loss function $\mathcal{L}_{b}$ to is more sensitive to small biomass number. In other words, given the same prediction error, the larger the biomass is, the less penalty the prediction network will receive. The relationship between error and regularized error can be found in Fig. \ref{fig:loss}.
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\columnwidth]{figs/loss_1.png}
    \caption{Graph showing the biomass prediction error regularized for different ground truth values.}
    \label{fig:loss}
\end{figure}

==> sec/4_experiment_05_11.tex <==
%%%%%%%%% BODY TEXT
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{sec:exp}
% The dataset to develop and validate our method was collected from a dryland cotton field experiment. The experiment was sown on a row spacing of 1 ${m}$ with a sowing density of ~10 plants ${m}^{2}$. A 'single skip' row sowing configuration was used (i.e., two rows planted, one row skipped). Each plot consisted of two sets of two 13 ${m}$ rows of cotton, with a 'skip' row in the middle of the plot and a shared skip row (with adjacent plots) on all borders of the plot. One set of two rows of cotton was used for non-destructive data collection, while the other set of two rows was used for destructive data collection.

% The experimental area (0.216 hectares) was scanned weekly with a drone flying 12 m above ground at a speed of 1.5 ${m/s}$. The drone captured a new image for every 4 m traveled. Biomass ground truth was collected on the day a flight was performed. We chose 9-time points, targeting key phenological plant stages during periods of high growth rate. 2 ${m}$ of above-ground plant material was cut at ground level from the 'destructive' data collection section of each plot. Plants were sampled from alternate rows up each plot to avoid any edge effects associated with reduced plant competition associated with previous biomass harvests. The number of plants and fresh weight were recorded. All sampled plants were then cut into ~50mm pieces and dried at 60 °C until no change in sample weight was observed ($\ge$ 48 h). 

\noindent \textbf{Dataset}: The dataset used to develop and validate our method was collected from a dryland cotton field experiment. It consisted of 24 plots and each plot contained two sets of two 13 ${m}$ cotton rows (2 kept intact throughout the season and 2 used for destructive ground truth measurements) spaced 1 ${m}$ apart, with a skip row in the middle and shared skip rows at plot borders. A drone surveyed the 0.216-hectare area weekly, flying 12 m above ground at 1.5 ${m/s}$ and capturing images every 4 ${m}$. Biomass ground truth was collected on 9 of the flight days, targeting key growth stages. In the 'destructive' data collection section of each plot, we cut 2 ${m}$ of above-ground material at ground level, sampling alternate rows to avoid edge effects. Plants were counted, fresh weighed, and subsequently dried at 60°C until weight stability was observed. Over the plant's life cycle (6 months) we therefore collected 216 (9 $\times$ 24) multi-view image sets with manually measured biomass ground truth. The dataset was split into 152 training sets and 64 testing sets. The 'Overall' testing set was split into 'Early Stage' (first 5 time points) and 'Late stage' (last 4 time points). Details of data collection and partition will be made available together with the dataset.

% \noindent \textbf{Implementations}: In our NeFF,  network ${F}_{g}$ is modeled by an MLP built by 8 hidden layers, and Relu with Softplus is used as the activation function for all hidden layers. A skip connection is used to connect the input and the fourth layer. The feature filed ${F}_{f}$ consists of an MLP with two hidden layers, while the color filed ${F}_{c}$ have four hidden layers. All hidden layers have the same hidden size of 256. Positional encoding is applied to spatial locations with 6 frequencies and viewing directions with 4 frequencies. We use 4 sparse 3D CNN blocks \ref{fig:3dbn} to compress the 3D features map into a 2D one, and the 3 Transformer encoders have the same defaulting as the original paper \cite{vaswani2017attention}. The final prediction MLP includes two hidden layers with 512 and 256 hidden sizes. We use an ADAM optimizer \cite{kingma2014adam} to optimize both networks on a Navida A5500 GPU. It takes 10 hours to optimize NeFF for 200K iterations, and around 8 hours to train Bionet for 100K iterations with 4 batchsize. 

\noindent \textbf{Implementations}: In our NeFF, ${F}_{g}$, ${F}_{f}$, and ${F}_{c}$ are modeled by an MLP with 8, 2, and 4 hidden layers, respectively (layer size=256). Positional encoding includes spatial locations with 6 frequencies and viewing directions with 4 frequencies. We used 4 sparse 3D CNN blocks and 5 Transformer encoders with the same defaulting as in  \cite{vaswani2017attention}. The final prediction MLP includes 2 hidden layers with 512 and 256 hidden sizes. We used ADAM \cite{kingma2014adam} to optimize NeFF (200k iteration, 512 rays) and Bionet (100k iterations, 4 batch sizes) on a Navida A5500.

% \noindent \textbf{Data Augmentation}: To reduce overfitting caused by training the complex model from scratch on a small dataset, we employ two data augmentation methods: rotation and motion. For rotation, each point extracted from the feature field is rotated around the origin [0,0,0] along the x, y, and z-axes by angles $\theta$, $\alpha$, and $\phi$, respectively. These angles are randomly sampled from the following ranges: $\theta \in \left[-\frac{\pi}{18}, \frac{\pi}{18}\right]$, $\alpha \in \left[-\frac{\pi}{18}, \frac{\pi}{18}\right]$, and $\phi \in \left[-\frac{\pi}{12}, \frac{\pi}{12}\right]$. As for motion, we introduce a translation offset $[\delta x, \delta y, \delta z]$ to shift all points along their corresponding axes. Each offset is independently sampled from a Gaussian distribution with a zero mean and unit standard deviation.
\noindent \textbf{Data Augmentation}: To prevent overfitting, we used two data augmentation methods: rotation and motion. Rotation involves random angle adjustments ($\theta$, $\alpha$, $\phi$) around x, y, z-axes within ranges ($\left[-\frac{\pi}{18}, \frac{\pi}{18}\right]$, $\left[-\frac{\pi}{18}, \frac{\pi}{18}\right]$, $\left[-\frac{\pi}{12}, \frac{\pi}{12}\right]$). Motion introduces Gaussian-distributed translation offsets ($\delta x, \delta y, \delta z$) with zero mean and unit standard deviation.

% \noindent \textbf{Baselines}: The currently widely-used biomass prediction method is the traditional density-based and non-learning method, i.e. 3DVI \cite{jimenez2018high, walter2019estimating}. Recently, there are also learning-based biomass prediction methods, such as PC-BioNet  \cite{pan2022biomass} proposed in 2022, but all these methods are based on point cloud. According to our knowledge, there is no multi-view-only and deep-learning-based biomass prediction network. To prove the effectiveness of our proposed method, we take as input the point cloud reconstructed by the structure-from-motion\cite{schonberger2016structure} for these point cloud-based biomass methods. Apart from that, we also add other SOTA point cloud learning methods, including PointNet\cite{qi2017pointnet}, PointNet++\cite{qi2017pointnet++}, and DGCNN \cite{wang2019dynamic}. We train these methods in our dataset (note: we haven't found other available dataset) and optimize them with the same optimizer and loss function.
\noindent \textbf{Baselines}: To test the performance of NeFF-BioNet, which is to our knowledge the first RGB multi-view and deep-learning-based biomass prediction network, we compared it to that of existing SOTA methods, namely 3DVI \cite{jimenez2018high, walter2019estimating} , BioNet (Referred to hereafter as PC-BioNet for Point Cloud-BioNet)  \cite{pan2022biomass}, PointNet\cite{qi2017pointnet}, PointNet++\cite{qi2017pointnet++}, and DGCNN \cite{wang2019dynamic}. Given that they all take point clouds as input, we used SfM~\cite{schonberger2016structure} to reconstruct point clouds from our RGB data and trained all methods on our dataset. We optimized all models with the same optimizer and loss function.

\noindent \textbf{Evaluation metrics}: We used similar metrics to evaluate biomass prediction errors as in \cite{pan2022biomass}, namely mean absolute error \textit{(MAE)}, mean absolute relative error (\textit{MARE}), and root mean square error \textit{(RMSE}). \textit{MARE} offers the advantage of being more robust against the range of ground truth values observed across our 9 times points.

\subsection{NeFF experiments}
\begin{figure}[htb]
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/Rendering_img.pdf}
    \caption{Rendering results showing a raw image (left), a rendered image (middle), and a rendered feature map (right). For visualization, the full feature map was compressed into 3 channels via a principal component analysis.}
    \label{fig:rendering}
\end{figure}
% We demonstrate the experimental results of the NeFF module in this section.
\noindent \textbf{Rendering} Examples of our image rendering can be found in Fig. \ref{fig:rendering}. We compared the rendering performance of our proposed method with that of NeuS\cite{NeuS_3D_reconstru}, a SOTA method which has a similar image rendering module to ours. The comparison results can be found in table \ref{tab:PSNR}. The quality of our novel view synthesis was evaluated in terms of peak signal-to-noise ratio (PSNR) and structural similarity index (SSIM). We observed that NeFF achieves similar performance in image rendering despite including two other tasks. This proves that the radiance field ${F}_{c}$, feature field ${F}_{f}$, and scene geometry modules ${F}_{g}$ are well decoupled, with each part trying to learn its own representation. We also observed that the NeFF without geometry loss $\mathcal{L}_{g}$ had a lower image rendering quality, the possible reason being that the scene geometry module ${F}_{g}$ with implicit supervision is simultaneously optimized by both the radiance and feature fields, and the feature field ${F}_{f}$ may have a negative effect on learning the radiance field ${F}_{c}$ via the geometry module ${F}_{g}$.

\begin{table}[h!]
    %\begin{adjustwidth}{-0.5cm}{}
    \centering
    \scalebox{0.85}{
    \begin{tabular}{c|c|c|c|c|c|c} 
    \specialrule{.1em}{.1em}{.1em}
    \multicolumn{2}{c|}{ Scene ID} & \#1 & \#3 & \#5 & \#7 & \#9 \\ \specialrule{.1em}{.1em}{.1em}
    \multirow{3}{*}{\centering PSNR$\uparrow$} & NeuS & 25.41 & \textbf{23.31} & 21.92 & \textbf{21.6} & 22.54  \\\cline{2-7}
    & w/o NeFF & 24.19 & 22.76 &  21.21 &  20.32& 22.05 \\ \cline{2-7}
    & NeFF & \textbf{25.86} & 23.09 & \textbf{22.03} & 20.99  & 22.76 \\ \specialrule{.1em}{.1em}{.1em}
    \multirow{3}{*}{\centering SSIM$\uparrow$} & NeuS   & 0.90 & \textbf{0.89} & 0.82& \textbf{0.82}& 0.85 \\\cline{2-7}
                                               & w/o NeFF & 0.84 & 0.81 & 0.79& 0.73& 0.83\\ \cline{2-7}
                                               & NeFF    & \textbf{0.92} & 0.87 & \textbf{0.84} & 0.77 &\textbf{0.86} \\ \hline
    \end{tabular}}
    %\end{adjustwidth}
    \caption{Quantitative comparison of our \textit{'NeFF'} method with NeuS on the task of novel-view image rendering on 1st, 3rd, 5th, 7th, and 9th time points. Rendering results of all image sets in a single time point were averaged. \textit{'w/o NeFF'} is our method without sparse point cloud supervision.}
    \label{tab:PSNR}
\end{table}


\noindent \textbf{3D reconstruction} Due to the complexity of collecting ground truth in a real-world scenario, our ground truth is limited in size and we consequently elected to evaluate the 3D reconstruction in our dataset qualitatively, as showed in Fig. \ref{fig:depth}. NeFF without sparse point cloud supervision leads to a rather flat and ambiguous 3D structure, whereas NeFF with sparse point cloud significantly improves the quality of 3D reconstructions, which can further enhance the quality of 3D feature representation.
\begin{table}[h!]
    %\begin{adjustwidth}{-0.0cm}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|c|c|c|c} 
    \specialrule{.1em}{.1em}{.1em}
    \multicolumn{2}{c|}{ Input} & MAE $\downarrow$ & MARE (\%) $\downarrow$ & RSME $\downarrow$ \\ \specialrule{.1em}{.1em}{.1em}
    \multirow{2}{*}{\centering w/o NeFF} &xyz & 235.9 &	0.497 &	383.4  \\\cline{2-5}
                                 & feature  & 220.6 & 0.464 & 349.5 \\ \specialrule{.1em}{.1em}{.1em}
    \multirow{2}{*}{\centering NeFF} & xyz  & 145.8	& 0.252	& 211.6 \\\cline{2-5}
                                 & feature  & \textbf{138.8} & \textbf{0.231} & \textbf{197.2} \\ \hline
    \end{tabular}}
    \caption{Ablation study on NeFF supervision and BioNet inputs. \textit{'w/o NeFF'} is our method without sparse point cloud supervision. \textit{'xyz'} and \textit{'feature'} represent BioNet inputs being either geometry coordinates or semantic features, respectively.}
    %\end{adjustwidth}
    
    \label{tab:feat_depth_sup}
\end{table}

\begin{figure}[htb]
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/depth.pdf}
    \caption{Visualization of 3D reconstruction showing a raw image (left), a 3D reconstruction with sparse point cloud supervision (middle), and a reconstruction without sparse point cloud supervision (right).}
    \label{fig:depth}
\end{figure}
% Provide convergence speed
% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figs/convergence.png}
%     \caption{The rendering convergence speed}
%     \label{fig:convergence}
%\end{figure}
\begin{table*}[h!]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{c c | c  c  c c c?c} \specialrule{.12em}{.12em}{.12em}
    \multicolumn{2}{c|}{\backslashbox{Metric}{Methods}} & PointNet\cite{qi2017pointnet} & PoinNet++\cite{qi2017pointnet++} & DGCNN\cite{wang2019dynamic} & PC-BioNet \cite{pan2022biomass} & 3DVI \cite{jimenez2018high} & Ours\\  \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Overall} \\ \hline
     \multirow{3}{*}{\centering Overall} & MAE $\downarrow$      & 177.2  & 166.2  & 156.7  & \underline{153.8}  & 206.2 & \textbf{138.8}  \\ % \cline{2-8}
      & MARE (\%) $\downarrow$& 0.32  & 0.311  & \underline{0.283}  & 0.292  & 0.428 &  \textbf{0.231}\\ % \cline{2-8}
      & RSME $\downarrow$     & 273.3  & 252.8  & 233.6  & \underline{228.4}  & 314.2 & \textbf{197.2}  \\  \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Early Stage} \\ \hline
     \multirow{3}{*}{\centering \makecell{Early \\ Stage}}  & MAE $\downarrow$ & 54.4 & 51.0& \underline{48.1}& 48.3& 63.3 & \textbf{42.8} \\ %\cline{2-8}
     &  MARE (\%) $\downarrow$& 0.358 & 0.348 & \underline{0.316} & 0.326& 0.478 & \textbf{0.262} \\ %\cline{2-8}
     &  RSME $\downarrow$& 84.1 & 77.8 & 71.9& \underline{70.3}& 96.7 & \textbf{61.7} \\  \specialrule{.12em}{.12em}{.12em}
     % \multicolumn{6}{c}{Late Stage} \\ \hline
     \multirow{3}{*}{\centering  \makecell{Late \\ Stage}}  & MAE $\downarrow$     & 231.5& 215.2& 211.2& \underline{191.4}& 267.8& \textbf{178.2} \\ %\cline{2-8}
     &  MARE (\%)$\downarrow$& 0.283& 0.276& 0.261& \underline{0.249} & 0.375& \textbf{0.197} \\ %\cline{2-8}
     &  RSME $\downarrow$    & 338.9& 311.8& 293.3& \underline{274.0}& 386.1& \textbf{241.7} \\  \specialrule{.12em}{.12em}{.12em}
    \end{tabular}}
    \caption{Quantitative performance comparisons of our proposed 'NeFF-BioNet' (Ours) with a range of SOTA methods; a volumetric method (3DVI) and various learning-based baselines (all others) - on our dataset. The best results are marked in \textit{\textbf{bold}}, and the second best results are \underline{underlined}. NeFF-BioNet was trained on the training dataset and evaluated on three different testing sets, i.e. 'Overall', 'Early Stage', and 'Late Stage'. The input for other SOTA methods is pseudo points obtained with SfM \cite{schonberger2016structure}. Our method achieves around 18\% overall accuracy gains compared to these methods.}
    \label{tab:exp_results}
\end{table*}

\begin{figure}[htb]
     \centering
     \includegraphics[width=0.75\columnwidth]{figs/number_encoder.png}
     \caption{Ablation study on the number of Transformer encoders in our BioNet module.}
     \label{fig:transformer_encoder}
\end{figure}


\subsection{Ablation experiments}
To demonstrate the contribution of various modules and types of information to the performance of our model, a number of ablation studies were performed over the whole dataset.

First we tested whether the use of the sparse point cloud supervision in NeFF could improve prediction accuracy. As shown in Table \ref{tab:feat_depth_sup}, it does lead to a 23.3\% improvement in MARE. Our dataset was captured in very flat and relatively textureless fields and this result demonstrates that explicit geometric supervision in NeFF is critical to biomass prediction in this context.  

We next tested whether the use of structural information (features) or geometrical coordinates (xyz) as input into BioNet yielded greater prediction accuracy. As seen in Table \ref{tab:feat_depth_sup}, 3D features indeed improved MARE by 2.1\%, suggesting that semantic features help BioNet to distinguish plants from foreground and background. Feature visualization can be found in Fig. \ref{fig:rendering} and supplementary material.

Finally, we conducted an ablation study on the number of Transformer encoders in BioNet (Fig. \ref{fig:transformer_encoder}). The 'zero' scenario corresponds to the absence of Transformers in the BioNet model. In this case the output of the sparse 3D backbone network is directly connected with the last two layers of the MLP for biomass prediction. The results of this experiment show that the prediction accuracy increases with $Num$ , then degrade slightly after $Num \ge 5$. This suggests that when the number of transformer encoders in BioNet is low, the biomass token cannot interact with other feature tokens well. When there are too many encoders, the Transformer module may overfit our dataset which results in degraded performance.

\subsection{Comparisons with other methods}
As mentioned in Sec. \ref{sec:exp}, we compared our proposed method with several baselines (Table \ref{tab:exp_results}). Namely, deep-learning-based methods (PointNet\cite{qi2017pointnet}, PointNet++\cite{qi2017pointnet++}, DGCNN \cite{wang2019dynamic}, and PC-BioNet \cite{pan2022biomass}), and a traditional density-based method (3DVI\cite{jimenez2018high}). All methods were trained on the entire dataset and evaluated on different testing sets: 'Early Stage', 'Late Stage', and 'Overall' (mix of both). From the result table, we can see that our proposed NeFF-BioNet achieves better biomass prediction accuracy than all baselines, showing around 18\%, 17\%, and 20\% relative MARE improvement over the second-best results on the 'Overall', 'Early Stage', and 'Late Stage' sets, respectively. The MAE and RSME of the 'Late Stage' set is much larger than that of the 'Early Stage' because crops in the late stages of their life cycle have much larger biomass than at early stages. We can also see that all methods perform better in the 'Late Stage' (lower MARE), possibly because crop structure can be better reconstructed by SfM~\cite{schonberger2016structure} as crops are bigger and show more distinguishable visual features. Amongst previous deep-learning-based methods, PC-BioNet performs similarly to DGCNN in 'Overall' and 'Early Stage' sets but outperforms DGCNN in the 'Late Stage' set. Both methods exhibit better prediction accuracy than PointNet and PointNet++. All deep-learning-based methods perform much better than the density-based method, 3DVI. This is possibly because here we are using pseudo point clouds rather than dense LiDAR point clouds used in \cite{pan2022biomass}, and the density-based method tends to be more sensitive to the quality of the point cloud than deep-learning-based methods. 




\begin{table*}[h!]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{c c | c  c  c c c?c} \specialrule{.12em}{.12em}{.12em}
    \multicolumn{2}{c|}{\backslashbox{Metric}{Methods}} & PointNet\cite{qi2017pointnet} & PoinNet++\cite{qi2017pointnet++} & DGCNN\cite{wang2019dynamic} & PC-BioNet \cite{pan2022biomass} & 3DVI \cite{jimenez2018high} & Ours\\  \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Overall} \\ \hline
     \multirow{3}{*}{\centering Overall} & MAE $\downarrow$ & 172.4 & 164.81 & 133.14 &  & & \textbf{120.94}  \\ % \cline{2-8}
      & MARE (\%) $\downarrow$& 0.253 & 0.229 & 0.236 & & & \textbf{0.174}\\ % \cline{2-8}
      & RSME $\downarrow$ & 256.3 & 215.55 & 203.57 & & & \textbf{180.11}  \\  \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Early Stage} \\ \hline
     \multirow{3}{*}{\centering \makecell{Early \\ Stage}}  & MAE $\downarrow$ &  &  &  &  &  & \textbf{35.7} \\ %\cline{2-8}
     &  MARE (\%) $\downarrow$& & & & & & \textbf{0.203} \\ %\cline{2-8}
     &  RSME $\downarrow$& & & & & &  \textbf{54.2}\\  \specialrule{.12em}{.12em}{.12em}
     % \multicolumn{6}{c}{Late Stage} \\ \hline
     \multirow{3}{*}{\centering  \makecell{Late \\ Stage}}  & MAE $\downarrow$&213.64&198.60 & & & & \textbf{163.5} \\ %\cline{2-8}
     &  MARE (\%)$\downarrow$&0.233 &0.222 & & & & \textbf{0.158} \\ %\cline{2-8}
     &  RSME $\downarrow$    &314.52& 295.50 & & & & \textbf{206.87} \\  \specialrule{.12em}{.12em}{.12em}
    \end{tabular}}
    \caption{Performance with LiDAR.}
    \label{tab:exp_results}
\end{table*}





\begin{table*}[h!]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{c  c | c  c  c c c?c} \specialrule{.12em}{.12em}{.12em}
    \multicolumn{2}{c|}{\backslashbox{Metric}{Methods}} & PointNet\cite{qi2017pointnet} & PoinNet++\cite{qi2017pointnet++} & DGCNN\cite{wang2019dynamic} & PC-BioNet \cite{pan2022biomass} & 3DVI \cite{jimenez2018high} & Ours\\  \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Overall} \\ \hline
     \multirow{3}{*}{\centering Overall} & MAE $\downarrow$ & 139.61 & 142.80 & 129.66 & 71.23 & 115.15 & \textbf{51.78}  \\ % \cline{2-8}
                                    & MARE (\%) $\downarrow$& 0.274 & 0.275 & 0.254 & 0.121 & 0.190 & \textbf{0.097}\\ % \cline{2-8}
                                            & RSME $\downarrow$ & 189.80 & 188.85 & 161.61 & 99.33 & 151.79 & \textbf{69.65}  \\  \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Early Stage} \\ \hline
     \multirow{3}{*}{\centering \makecell{Early \\ Stage}}& MAE $\downarrow$& 92.59 &120.62 & 83.07 &43.11&60.45 & \textbf{35.06}\\ %\cline{2-8}
                                                        &  MARE(\%) $\downarrow$& 0.326 &0.411 & 0.334 &0.135 &0.211 & \textbf{0.121}\\ %\cline{2-8}
                                                            &  RSME $\downarrow$& 108.5 &159.17 &98.67 &57.71 &69.83 &  \textbf{42.33}\\  \specialrule{.12em}{.12em}{.12em}
     % \multicolumn{6}{c}{Late Stage} \\ \hline
     \multirow{3}{*}{\centering  \makecell{Late \\ Stage}}  & MAE $\downarrow$&188.52 &181.69 &170.10 &100.47 &172.04 & \textbf{62.41} \\ %\cline{2-8}
                                                      &  MARE (\%)$\downarrow$&0.219 &0.179 &0.164 &0.106 &0.168 & \textbf{0.066} \\ %\cline{2-8}
                                                          &  RSME $\downarrow$&247.48 &230.96 &207.74 &129.09 &204.77 & \textbf{84.30} \\  \specialrule{.12em}{.12em}{.12em}
    \end{tabular}}
    \caption{Performance with wheat Dataset.}
    \label{tab:exp_results}
\end{table*}





\begin{table*}[h!]
    \centering
    \scalebox{0.9}{
    
    \begin{tabular}{c  c | c c c c |c c  c c } \specialrule{.12em}{.12em}{.12em}
    
    \multicolumn{2}{c|}{\multirow{2}{*}{\backslashbox{Training}{Testing}}}& \multicolumn{4}{ c}{ Early stage } & \multicolumn{4}{|c}{ Flowering stage } \\  
    \multicolume{}{}{} & & DGCNN  & PC-BioNet & 3DVI & Ours & DGCNN & PC-BioNet & 3DVI & Ours\\ \specialrule{.12em}{.12em}{.12em}

    \multirow{3}{*}{ Early stage } & MAE $\downarrow$ & 101.75  & 50.53 &  53.82 & \textbf{34.80} & 592.91 & 121.86 & \textbf{109.57}  & 130.76\\
    & MARE (\%) $\downarrow$ & 0.247 & 0.134 & 0.168 & \textbf{0.124} & 0.658 & 0.137 & \textbf{0.114} & 0.158\\
    & RMSE $\downarrow$ & 116.05 & 62.18 & 66.71 & \textbf{43.29} & 613.57 & 226.45 & \textbf{186.31} & 242.6\\ \specialrule{.12em}{.12em}{.12em}
    \multirow{3}{*}{ Flowering stage } & MAE $\downarrow$ & 563.11& 114.46 & \textbf{62.14}  &102.62 & 133.28 & 111.13 & 102.97  & \textbf{58.58} \\
    & MARE (\%) $\downarrow$ & 1.476 & 0.295  & \textbf{0.163} & 0.262 & 0.115& 0.099 & 0.109  & \textbf{0.063} \\
    & RMSE $\downarrow$ & 566.32& 124.46 & \textbf{74.75}  & 112.78 & 150.15 & 145.65  & 129.45 & \textbf{80.21}\\ \specialrule{.12em}{.12em}{.12em}
    
    \end{tabular}
    }
    \caption{Generalization capability.}
    \label{tab:exp_results}
\end{table*}


==> sec/4_experiment_18_11.tex <==
%%%%%%%%% BODY TEXT
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{sec:exp}

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/wc_vis.png}
    \caption{Visualization of a point cloud of publicly available wheat biomass dataset (right) and our self-collected dataset (left).}
    \label{fig:pc_vis}
\end{figure}


% The dataset to develop and validate our method was collected from a dryland cotton field experiment. The experiment was sown on a row spacing of 1 ${m}$ with a sowing density of ~10 plants ${m}^{2}$. A 'single skip' row sowing configuration was used (i.e., two rows planted, one row skipped). Each plot consisted of two sets of two 13 ${m}$ rows of cotton, with a 'skip' row in the middle of the plot and a shared skip row (with adjacent plots) on all borders of the plot. One set of two rows of cotton was used for non-destructive data collection, while the other set of two rows was used for destructive data collection.

% The experimental area (0.216 hectares) was scanned weekly with a drone flying 12 m above ground at a speed of 1.5 ${m/s}$. The drone captured a new image for every 4 m traveled. Biomass ground truth was collected on the day a flight was performed. We chose 9-time points, targeting key phenological plant stages during periods of high growth rate. 2 ${m}$ of above-ground plant material was cut at ground level from the 'destructive' data collection section of each plot. Plants were sampled from alternate rows up each plot to avoid any edge effects associated with reduced plant competition associated with previous biomass harvests. The number of plants and fresh weight were recorded. All sampled plants were then cut into ~50mm pieces and dried at 60 °C until no change in sample weight was observed ($\ge$ 48 h). 

\noindent \textbf{Dataset}: The dataset used to develop and validate our method was collected from a dryland cotton field experiment. It consisted of 24 plots and each plot contained two sets of two 13 ${m}$ cotton rows. We chose 9-time points, targeting the key growth stage, and used the drone camera and LiDAR to scan the field at each time point. Biomass ground truth was collected on the same day of data collection. In total, we collected 216 (9 $\times$ 24) multi-view image sets with LiDAR point cloud and manually measured biomass ground truth. The dataset was split into 152 training sets and 64 testing sets. Details of data collection and partition can be found in the supplementary and the dataset will be made publicly available. The comparison between our dataset and another biomass dataset can be found in Table \ref{tab:dataset_comparison} and Fig. \ref{fig:pc_vis}.


\begin{table}[h!]
    \centering
    \scalebox{0.75}{
    \begin{tabular}{c|c|c|c} 
    \specialrule{.1em}{.1em}{.1em}
    Dataset name & Modality & Number of Plot & Plot size (m\textsuperscript{2}) \\ \hline
    Ours  & Camera and LiDAR & 216 & 1$\times$15 \\ \hline
    PC-BioNet \cite{pan2022biomass} & LiDAR & 306 & 1$\times$1 \\ \hline
    \end{tabular}
    }
    \caption{Dataset comparison}
    \label{tab:dataset_comparison}
\end{table}



% \noindent \textbf{Implementations}: In our NeFF,  network ${F}_{g}$ is modeled by an MLP built by 8 hidden layers, and Relu with Softplus is used as the activation function for all hidden layers. A skip connection is used to connect the input and the fourth layer. The feature filed ${F}_{f}$ consists of an MLP with two hidden layers, while the color filed ${F}_{c}$ have four hidden layers. All hidden layers have the same hidden size of 256. Positional encoding is applied to spatial locations with 6 frequencies and viewing directions with 4 frequencies. We use 4 sparse 3D CNN blocks \ref{fig:3dbn} to compress the 3D features map into a 2D one, and the 3 Transformer encoders have the same defaulting as the original paper \cite{vaswani2017attention}. The final prediction MLP includes two hidden layers with 512 and 256 hidden sizes. We use an ADAM optimizer \cite{kingma2014adam} to optimize both networks on a Navida A5500 GPU. It takes 10 hours to optimize NeFF for 200K iterations, and around 8 hours to train Bionet for 100K iterations with 4 batchsize. 


% \noindent \textbf{Data Augmentation}: To reduce overfitting caused by training the complex model from scratch on a small dataset, we employ two data augmentation methods: rotation and motion. For rotation, each point extracted from the feature field is rotated around the origin [0,0,0] along the x, y, and z-axes by angles $\theta$, $\alpha$, and $\phi$, respectively. These angles are randomly sampled from the following ranges: $\theta \in \left[-\frac{\pi}{18}, \frac{\pi}{18}\right]$, $\alpha \in \left[-\frac{\pi}{18}, \frac{\pi}{18}\right]$, and $\phi \in \left[-\frac{\pi}{12}, \frac{\pi}{12}\right]$. As for motion, we introduce a translation offset $[\delta x, \delta y, \delta z]$ to shift all points along their corresponding axes. Each offset is independently sampled from a Gaussian distribution with a zero mean and unit standard deviation.
\noindent \textbf{Data Augmentation}: To prevent overfitting, we used two data augmentation methods: rotation and motion. Rotation involves random angle adjustments ($\theta$, $\alpha$, $\phi$) around x, y, z-axes within ranges ($\left[-\frac{\pi}{18}, \frac{\pi}{18}\right]$, $\left[-\frac{\pi}{18}, \frac{\pi}{18}\right]$, $\left[-\frac{\pi}{12}, \frac{\pi}{12}\right]$). Motion introduces Gaussian-distributed translation offsets ($\delta x, \delta y, \delta z$) with zero mean and unit standard deviation.

% \noindent \textbf{Baselines}: The currently widely-used biomass prediction method is the traditional density-based and non-learning method, i.e. 3DVI \cite{jimenez2018high, walter2019estimating}. Recently, there are also learning-based biomass prediction methods, such as PC-BioNet  \cite{pan2022biomass} proposed in 2022, but all these methods are based on point cloud. According to our knowledge, there is no multi-view-only and deep-learning-based biomass prediction network. To prove the effectiveness of our proposed method, we take as input the point cloud reconstructed by the structure-from-motion\cite{schonberger2016structure} for these point cloud-based biomass methods. Apart from that, we also add other SOTA point cloud learning methods, including PointNet\cite{qi2017pointnet}, PointNet++\cite{qi2017pointnet++}, and DGCNN \cite{wang2019dynamic}. We train these methods in our dataset (note: we haven't found other available dataset) and optimize them with the same optimizer and loss function.
\noindent \textbf{Baselines}: To test the performance of NeFF-BioNet, which is to our knowledge the first RGB multi-view and deep-learning-based biomass prediction network, we compared it to that of existing SOTA methods, namely 3DVI \cite{jimenez2018high, walter2019estimating} , BioNet (Referred to hereafter as PC-BioNet for Point Cloud-BioNet)  \cite{pan2022biomass}, PointNet\cite{qi2017pointnet}, PointNet++\cite{qi2017pointnet++}, and DGCNN \cite{wang2019dynamic}. Given that they all take point clouds as input, we used SfM~\cite{schonberger2016structure} to reconstruct point clouds from our RGB data and trained all methods on our dataset. We optimized all models with the same optimizer and loss function.

\noindent \textbf{Evaluation metrics}: We used similar metrics to evaluate biomass prediction errors as in \cite{pan2022biomass}, namely mean absolute error \textit{(MAE)}, mean absolute relative error (\textit{MARE}), and root mean square error \textit{(RMSE}). \textit{MARE} offers the advantage of being more robust against the range of ground truth values observed across our 9 times points.

\subsection{NeFF experiments}
\begin{figure}[htb]
    \centering
    \includegraphics[width=.8\columnwidth]{figs/Rendering_img.pdf}
    \caption{Rendering results showing a raw image (left), a rendered image (middle), and a rendered feature map (right). Full feature maps were compressed into 3 channels via PCA for visualization.}
    \label{fig:rendering}
\end{figure}
% We demonstrate the experimental results of the NeFF module in this section.
\noindent \textbf{Rendering} Examples of our image rendering can be found in Fig. \ref{fig:rendering}. We compared the rendering performance of our proposed method with that of NeuS\cite{NeuS_3D_reconstru}, a SOTA method which has a similar image rendering module to ours. The comparison results can be found in table \ref{tab:PSNR}. The quality of our novel view synthesis was evaluated in terms of peak signal-to-noise ratio (PSNR) and structural similarity index (SSIM). We observed that NeFF achieves similar performance in image rendering despite including two other tasks. This proves that the radiance field ${F}_{c}$, feature field ${F}_{f}$, and scene geometry modules ${F}_{g}$ are well decoupled, with each part trying to learn its own representation. We also observed that the NeFF without geometry loss $\mathcal{L}_{g}$ had a lower image rendering quality, the possible reason being that the scene geometry module ${F}_{g}$ with implicit supervision is simultaneously optimized by both the radiance and feature fields, and the feature field ${F}_{f}$ may have a negative effect on learning the radiance field ${F}_{c}$ via the geometry module ${F}_{g}$.

\begin{table}[h!]
    %\begin{adjustwidth}{-0.5cm}{}
    \centering
    \scalebox{0.85}{
    \begin{tabular}{c|c|c|c|c|c|c} 
    \specialrule{.1em}{.1em}{.1em}
    \multicolumn{2}{c|}{ Scene ID} & \#1 & \#3 & \#5 & \#7 & \#9 \\ \specialrule{.1em}{.1em}{.1em}
    \multirow{3}{*}{\centering PSNR$\uparrow$} & NeuS & 25.41 & \textbf{23.31} & 21.92 & \textbf{21.6} & 22.54  \\\cline{2-7}
    & w/o NeFF & 24.19 & 22.76 &  21.21 &  20.32& 22.05 \\ \cline{2-7}
    & NeFF & \textbf{25.86} & 23.09 & \textbf{22.03} & 20.99  & 22.76 \\ \specialrule{.1em}{.1em}{.1em}
    \multirow{3}{*}{\centering SSIM$\uparrow$} & NeuS   & 0.90 & \textbf{0.89} & 0.82& \textbf{0.82}& 0.85 \\\cline{2-7}
                                               & w/o NeFF & 0.84 & 0.81 & 0.79& 0.73& 0.83\\ \cline{2-7}
                                               & NeFF    & \textbf{0.92} & 0.87 & \textbf{0.84} & 0.77 &\textbf{0.86} \\ \hline
    \end{tabular}}
    %\end{adjustwidth}
    \caption{Quantitative comparison of our \textit{'NeFF'} method with NeuS on the task of novel-view image rendering on 1st, 3rd, 5th, 7th, and 9th time points. Rendering results of all image sets in a single time point were averaged. \textit{'w/o NeFF'} is our method without sparse point cloud supervision.}
    \label{tab:PSNR}
\end{table}


\noindent \textbf{3D reconstruction} Due to the complexity of collecting ground truth in a real-world scenario, our ground truth is limited in size and we consequently elected to evaluate the 3D reconstruction in our dataset qualitatively, as showed in Fig. \ref{fig:depth}. NeFF without sparse point cloud supervision leads to a rather flat and ambiguous 3D structure, whereas NeFF with sparse point cloud significantly improves the quality of 3D reconstructions, which can further enhance the quality of 3D feature representation.
\begin{table}[h!]
    %\begin{adjustwidth}{-0.0cm}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|c|c|c|c} 
    \specialrule{.1em}{.1em}{.1em}
    \multicolumn{2}{c|}{ Input} & MAE $\downarrow$ & MARE (\%) $\downarrow$ & RSME $\downarrow$ \\ \specialrule{.1em}{.1em}{.1em}
    \multirow{2}{*}{\centering w/o NeFF} &xyz & 235.9 &	0.497 &	383.4  \\\cline{2-5}
                                 & feature  & 220.6 & 0.464 & 349.5 \\ \specialrule{.1em}{.1em}{.1em}
    \multirow{2}{*}{\centering NeFF} & xyz  & 145.8	& 0.252	& 211.6 \\\cline{2-5}
                                 & feature  & \textbf{138.8} & \textbf{0.231} & \textbf{197.2} \\ \hline
    \end{tabular}}
    \caption{Ablation study on NeFF supervision and BioNet inputs. \textit{'w/o NeFF'} is our method without sparse point cloud supervision. \textit{'xyz'} and \textit{'feature'} represent BioNet inputs being either geometry coordinates or semantic features, respectively.}
    %\end{adjustwidth}
    
    \label{tab:feat_depth_sup}
\end{table}

\begin{figure}[htb]
    \centering
    \includegraphics[width=1.0\columnwidth]{figs/depth.pdf}
    \caption{Visualization of 3D reconstruction showing a raw image (left), a 3D reconstruction with sparse point cloud supervision (middle), and a reconstruction without sparse point cloud supervision (right).}
    \label{fig:depth}
\end{figure}
% Provide convergence speed
% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figs/convergence.png}
%     \caption{The rendering convergence speed}
%     \label{fig:convergence}
%\end{figure}
\begin{table*}[h!]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{c c | c  c  c c c  c} 
    \specialrule{.12em}{.12em}{.12em}
    \multicolumn{2}{c|}{\backslashbox{Metric}{Methods}} & PointNet\cite{qi2017pointnet} & PoinNet++\cite{qi2017pointnet++} & DGCNN\cite{wang2019dynamic} & PC-BioNet \cite{pan2022biomass} & 3DVI \cite{jimenez2018high} & Ours\\
    \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Overall} \\ \hline
     \multirow{3}{*}{\makecell{Image}} & MAE $\downarrow$ & 177.2  & 166.2  & 156.7  & \underline{153.8}  & 206.2 & \textbf{138.8}  \\ % \cline{2-8}
      & MARE $\downarrow$& 0.32  & 0.311  & \underline{0.283}  & 0.292  & 0.428 &  \textbf{0.231}\\ % \cline{2-8}
      & RSME $\downarrow$     & 273.3  & 252.8  & 233.6  & \underline{228.4}  & 314.2 & \textbf{197.2}  \\  \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Early Stage} \\ \hline
     \multirow{3}{*}{\makecell{Point \\ cloud}} & MAE $\downarrow$ & 172.4 & 164.81 & 133.14 &  \underline{128.76}  &  130.34 & \textbf{120.94}  \\ % \cline{2-8}
      & MARE $\downarrow$& 0.253 & 0.229 & 0.236 &  \underline{0.201} & 0.225 & \textbf{0.174}\\ % \cline{2-8}
      & RSME $\downarrow$ & 256.3 & 215.55 & 203.57 &  \underline{194.51} & 204.83 & \textbf{180.11}  \\  \specialrule{.12em}{.12em}{.12em}
    \end{tabular}}
    \caption{Quantitative performance comparisons of our proposed 'NeFF-BioNet' (Ours) with a range of SOTA methods; a volumetric method (3DVI) and various learning-based baselines (all others) - on our dataset. The best results are marked in \textit{\textbf{bold}}, and the second best results are \underline{underlined}. NeFF-BioNet was trained on the training dataset and evaluated on three different testing sets, i.e. 'Overall', 'Early Stage', and 'Late Stage'. The input for other SOTA methods is pseudo points obtained with SfM \cite{schonberger2016structure}. Our method achieves around 18\% overall accuracy gains compared to these methods.}
    \label{tab:exp_results}
\end{table*}






\begin{figure}[htb]
     \centering
     \includegraphics[width=0.75\columnwidth]{figs/number_encoder.png}
     \caption{Ablation study on the number of Transformer encoders in our BioNet module.}
     \label{fig:transformer_encoder}
\end{figure}


\subsection{Ablation experiments}
To demonstrate the contribution of various modules and types of information to the performance of our model, a number of ablation studies were performed over the whole dataset.

First we tested whether the use of the sparse point cloud supervision in NeFF could improve prediction accuracy. As shown in Table \ref{tab:feat_depth_sup}, it does lead to a 23.3\% improvement in MARE. Our dataset was captured in very flat and relatively textureless fields and this result demonstrates that explicit geometric supervision in NeFF is critical to biomass prediction in this context.  

We next tested whether the use of structural information (features) or geometrical coordinates (xyz) as input into BioNet yielded greater prediction accuracy. As seen in Table \ref{tab:feat_depth_sup}, 3D features indeed improved MARE by 2.1\%, suggesting that semantic features help BioNet to distinguish plants from foreground and background. Feature visualization can be found in Fig. \ref{fig:rendering} and supplementary material.

Finally, we conducted an ablation study on the number of Transformer encoders in BioNet (Fig. \ref{fig:transformer_encoder}). The 'zero' scenario corresponds to the absence of Transformers in the BioNet model. In this case the output of the sparse 3D backbone network is directly connected with the last two layers of the MLP for biomass prediction. The results of this experiment show that the prediction accuracy increases with $Num$ , then degrade slightly after $Num \ge 5$. This suggests that when the number of transformer encoders in BioNet is low, the biomass token cannot interact with other feature tokens well. When there are too many encoders, the Transformer module may overfit our dataset which results in degraded performance.

\subsection{Comparisons with other methods}
As mentioned in Sec. \ref{sec:exp}, we compared our proposed method with several baselines (Table \ref{tab:exp_results}). Namely, deep-learning-based methods (PointNet\cite{qi2017pointnet}, PointNet++\cite{qi2017pointnet++}, DGCNN \cite{wang2019dynamic}, and PC-BioNet \cite{pan2022biomass}), and a traditional density-based method (3DVI\cite{jimenez2018high}). All methods were trained on the entire dataset and evaluated on different testing sets: 'Early Stage', 'Late Stage', and 'Overall' (mix of both). From the result table, we can see that our proposed NeFF-BioNet achieves better biomass prediction accuracy than all baselines, showing around 18\%, 17\%, and 20\% relative MARE improvement over the second-best results on the 'Overall', 'Early Stage', and 'Late Stage' sets, respectively. The MAE and RSME of the 'Late Stage' set is much larger than that of the 'Early Stage' because crops in the late stages of their life cycle have much larger biomass than at early stages. We can also see that all methods perform better in the 'Late Stage' (lower MARE), possibly because crop structure can be better reconstructed by SfM~\cite{schonberger2016structure} as crops are bigger and show more distinguishable visual features. Amongst previous deep-learning-based methods, PC-BioNet performs similarly to DGCNN in 'Overall' and 'Early Stage' sets but outperforms DGCNN in the 'Late Stage' set. Both methods exhibit better prediction accuracy than PointNet and PointNet++. All deep-learning-based methods perform much better than the density-based method, 3DVI. This is possibly because here we are using pseudo point clouds rather than dense LiDAR point clouds used in \cite{pan2022biomass}, and the density-based method tends to be more sensitive to the quality of the point cloud than deep-learning-based methods. 




\begin{table*}[h!]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{c  c | c  c  c c c c} \specialrule{.12em}{.12em}{.12em}
    \multicolumn{2}{c|}{\backslashbox{Metric}{Methods}} & PointNet\cite{qi2017pointnet} & PoinNet++\cite{qi2017pointnet++} & DGCNN\cite{wang2019dynamic} & PC-BioNet \cite{pan2022biomass} & 3DVI \cite{jimenez2018high} & Ours\\  \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Overall} \\ \hline
     \multirow{3}{*}{\makecell{Overall}} & MAE $\downarrow$ & 139.61 & 142.80 & 129.66 & 71.23 & 115.15 & \textbf{51.78}  \\ % \cline{2-8}
                                    & MARE $\downarrow$& 0.274 & 0.275 & 0.254 & 0.121 & 0.190 & \textbf{0.097}\\ % \cline{2-8}
                                            & RSME $\downarrow$ & 189.80 & 188.85 & 161.61 & 99.33 & 151.79 & \textbf{69.65}  \\  \specialrule{.12em}{.12em}{.12em}
    % \multicolumn{6}{c}{Early Stage} \\ \hline
     \multirow{3}{*}{\centering \makecell{Early \\ Stage}}& MAE $\downarrow$& 92.59 &120.62 & 83.07 &43.11&60.45 & \textbf{35.06}\\ %\cline{2-8}
                                                        & MARE $\downarrow$& 0.326 &0.411 & 0.334 &0.135 &0.211 & \textbf{0.121}\\ %\cline{2-8}
                                                        &  RSME $\downarrow$& 108.5 &159.17 &98.67 &57.71 &69.83 &  \textbf{42.33}\\  \specialrule{.12em}{.12em}{.12em}
     % \multicolumn{6}{c}{Late Stage} \\ \hline
     \multirow{3}{*}{\centering  \makecell{Late \\ Stage}}  & MAE $\downarrow$&188.52 &181.69 &170.10 &100.47 &172.04 & \textbf{62.41} \\ %\cline{2-8}
                                                      &  MARE $\downarrow$&0.219 &0.179 &0.164 &0.106 &0.168 & \textbf{0.066} \\ %\cline{2-8}
                                                      &  RSME $\downarrow$&247.48 &230.96 &207.74 &129.09 &204.77 & \textbf{84.30} \\  \specialrule{.12em}{.12em}{.12em}
    \end{tabular}}
    \caption{Performance with wheat Dataset.}
    \label{tab:exp_results}
\end{table*}



\begin{table*}[h!]
    \centering
    \scalebox{0.9}{
    
    \begin{tabular}{c  c | c c c |c c c } \specialrule{.12em}{.12em}{.12em}
    
    \multicolumn{2}{c|}{\multirow{2}{*}{\backslashbox{Training}{Testing}}}& \multicolumn{3}{ c}{ Early stage } & \multicolumn{3}{|c}{ Flowering stage } \\  
    \multicolume{}{}{} & & DGCNN~\cite{wang2019dynamic}  & PC-BioNet~\cite{pan2022biomass} & Ours & DGCNN~\cite{wang2019dynamic} & PC-BioNet~\cite{pan2022biomass} & Ours\\ \specialrule{.12em}{.12em}{.12em}

    \multirow{3}{*}{ Early stage } & MAE $\downarrow$ & 101.75  & 50.53 &  \textbf{34.80} & 592.91 & \textbf{121.86} &  130.76\\
    & MARE $\downarrow$ & 0.247 & 0.134 & \textbf{0.124} & 0.658 & \textbf{0.137} & 0.158\\
    & RMSE $\downarrow$ & 116.05 & 62.18 & \textbf{43.29} & 613.57 & \textbf{226.45} & 242.6\\ \specialrule{.12em}{.12em}{.12em}
    \multirow{3}{*}{ Flowering stage } & MAE $\downarrow$ & 563.11& 114.46 & \textbf{62.14}  &102.62 & 133.28 & \textbf{58.58} \\
    & MARE $\downarrow$ & 1.476 & 0.295  & \textbf{0.163} & 0.262 & 0.115& \textbf{0.063} \\
    & RMSE $\downarrow$ & 566.32& 124.46 & \textbf{74.75}  & 112.78 & 150.15 & \textbf{80.21}\\ \specialrule{.12em}{.12em}{.12em}
    
    \end{tabular}
    }
    \caption{Generalization capability.}
    \label{tab:exp_results}
\end{table*}

